Improving Count-Mean Sketch as the Leading Locally Differentially Private Frequency Estimator for Large Dictionaries

This paper identifies that a group of latest locally-differentially-private (LDP) algorithms for frequency estimation, including all the Hadamard-matrix-based algorithms, are equivalent to the private Count-Mean Sketch (CMS) algorithm with different parameters. Therefore, we revisit the private CMS, correct errors in the original CMS paper regarding expectation and variance, modify the CMS implementation to eliminate existing bias, and optimize CMS using randomized response (RR) as the perturbation method. The optimized CMS with RR is shown to outperform CMS variants with other known perturbations in reducing the worst-case mean squared error (MSE), $l_1$ loss, and $l_2$ loss. Additionally, we prove that pairwise-independent hashing is sufficient for CMS, reducing its communication cost to the logarithm of the cardinality of all possible values (i.e., a dictionary). As a result, the optimized CMS with RR is proven theoretically and empirically as the leading algorithm for reducing the aforementioned loss functions when dealing with a very large dictionary. Furthermore, we demonstrate that randomness is necessary to ensure the correctness of CMS, and the communication cost of CMS, though low, is unavoidable despite the randomness being public or private.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> unused.tex <==
Eq. \eqref{eq:a_i_F_i} can always be rewritten as the linear combination of at most $L$ other independent equations, each in form of

\begin{equation}
  \sum_{i \in \phi_j} F_i = \sum_{i' \in \psi_j} F_{i'} , 
  \label{eq:F_i=F_i}
\end{equation}

\noindent where $j$ indexes the $j$-th independent equation. Thus, Eq. \eqref{eq:a_i_F_i} can be rewritten as

\begin{equation}
    \sum_{j \in [k]} b_j \sum_{i \in \phi_j} F_i = \sum_{j \in [k]} b_j \sum_{i' \in \psi_j} F_{i'} ,
\end{equation}
 
\noindent where $k$ is reused as the number of independent equations needed to reconstruct Eq. \eqref{eq:a_i_F_i}. Subsequently, for each Eq. \eqref{eq:F_i=F_i} above, we can apply Eq. \eqref{eq:another_v} accordingly to update $\mathbf{v}$. If the updated $\mathbf{v}'$ is always similar to $\mathbf{v}$, we can say this system still has a nearly-unique solution. In the following section, we will only focus on the equations in the form of Eq. \eqref{eq:F_i=F_i} for simplicity, but the conclusion will be applicable to any equations in the form of Eq. \eqref{eq:a_i_F_i}.

Given a filter $F$, if all the Eq. \eqref{eq:F_i=F_i} satisfied by $F$ have $|\phi| > M$, and $\mathbf{v}$ has at most $M$ non-negative values, then there will be no way to construct an alternative $\mathbf{v}'$, because at least one $v_i$ whose $i \in \phi$ will be negative after applying $v'_i = v_i + \Delta$.

 Suppose for any such relationship in a system, if at least one $v_i < \theta$, then there will be no corresponding $v_j \ge \theta$. Therefore all the solutions of the system will be similar.

Now the question is how to form a Bloom-filter mapping that prevents the existence of such a relationship.



On the other hand, if the public allocation is unchanged every time the CMS is run, one can always construct a counterexample making $Var_{\forall j: c_j(x, x')}( E[\hat{f}(x)] )$ independent of $k$, meaning that adding more hash functions will not reduce the bias of the expectation. Since $(X^{(i)})_{i \in [n]}$ are allowed to be arbitrary values, we can set value $j$ to the object being assigned to the $j$-th hash function. Then, we will have $\sum_{j \in [k]} n_j(x')^2 = n(x')^2$ for any $x'$, which leads to

\begin{equation*}
    Var_{\forall j: c_j(x, x')}( E[\hat{f}(x)] ) = \frac{1}{m - 1} \sum_{x' \in [k] \backslash x} f(x')^2 ,
\end{equation*}

\noindent where $f(x')$ is the frequency of value $x'$. We can see the variance remains the same even when $k$ increases significantly. An example of a deterministic public allocation among different runs is X, which proposed to assign the hash functions to objects in a round-robin way. 


\section{Optimized CMS}

For Eq. \eqref{eq:optimized_cms_var_rr_half_done}, when

\begin{equation}
    m =  \frac{ \Delta }{f(x) (e^{\epsilon} - 1) + 1} + 1 , \notag
\end{equation}

\noindent where
\begin{equation}
    \Delta = \sqrt{ [f(x) (e^{\epsilon} - 1) + 1] [2 e^{\epsilon} - f(x) (e^{\epsilon} - 1) - 1 ] } , \notag
\end{equation}

\noindent $Var(\hat{f}(x))$ is minimized as

\begin{multline}
        Var^*(\hat{f}(x))_{RR} = \\ \frac{ [ f(x)(e^{\epsilon} - 1) + 1 + \Delta ] [2 e^{\epsilon} - f(x) (e^{\epsilon} - 1) - 1 + \Delta ]   }{n \Delta  (e^{\epsilon} - 1)^2 } \\ =
        \frac{2 \Delta + 2 e^{\epsilon} }{n (e^{\epsilon} - 1)^2  }.
    \label{eq:optimized_cms_var_rr}
\end{multline}

If deriving $Var(\hat{f}(x))_{OUE}$ by $m$, we will find its derivative as negative. Thus, it decreases when $m$ increases. When $m$ is large enough, we have

\begin{equation}
    Var(\hat{f}(x))_{OUE} \rightarrow \frac{f(x) (e^{\epsilon} - 1)^2 + 4  e^{\epsilon} }{ n (e^{\epsilon} - 1)^2} .
\end{equation}

However, plotting the minimum of $Var(\hat{f}(x))_{RR}$ vs $Var(\hat{f}(x))_{OUE}$, we will see $Var(\hat{f}(x))_{RR} < Var(\hat{f}(x))_{OUE}$ for all $\epsilon > 0$. Thus, the optimized CMS uses the randomized response to process the hashed values, and set $m$ to be the integer close to $\frac{ \Delta }{f(x) (e^{\epsilon} - 1) + 1} + 1$. Since deploying randomized responses is always preferred, we will abbreviate $Var^*(\hat{f}(x))_{RR}$ as $Var^*(\hat{f}(x))$. We will discuss how to handle $f(x)$ later.

We observe that $\frac{\partial \Delta}{\partial f(x)} \ge 0$ when $0 \le f(x) \le 1$, implying that $\Delta$ increases monotonically in this range, so does $Var^*(\hat{f}(x))_{RR}$. If we aim to minimize the $l_{\infty}$, which is equivalent to reducing the worst-case variance, we should consider the case where $f(x) = 1$:

\begin{equation}
    l_{\infty} = \max_{f(x)} Var^*(\hat{f}(x)) = \frac{4 e^{\epsilon}}{(e^{\epsilon} - 1)^2} , \notag
\end{equation}

\noindent and $m = 2$.

On the other hand, observe the $l_2$ loss with significant candidates:
\begin{equation}
    l_2 = \sum_{x \in [d^*]}  Var^*(\hat{f}(x)) = 
\end{equation}


For $l_1$ loss of an unbiased estimator of $f(x)$, given that $E[\sqrt{X}] \le \sqrt{E[X]}$, we have
\begin{multline}
    l_1 = E[\sum_{x \in [d]} | \hat{f}(x) - f(x)|] \\ = \sum_{x \in [d]} E[\sqrt{( \hat{f}(x) - f(x) )^2}] \le  \sum_{x \in [d]} \sqrt{Var(\hat{f}(x))} ,
\end{multline}

Notice that $Var(\hat{f}(x))$ is a linear function of $f(x)$, so $\sqrt{Var(\hat{f})(x)}$ becomes a concave function of $f(x)$, and we have
\begin{multline}
    l_1 \le  d \sqrt{Var \bigl( \hat{f}(x) | f(x) = \frac{\sum_{x' \in [d]} f(x')}{d}} \bigr) \\ =  d \sqrt{Var \bigl( \hat{f}(x) | f(x) = \frac{1}{d}} \bigr).
\end{multline}

When using randomized response to perturb the hashed values, we have
\begin{multline}
    l_{1, RR} \le \\ d \sqrt{ \frac{ (d + e^{\epsilon} - 1) m^2}{n (m - 1) (e^{\epsilon} - 1)^2}  +  \frac{   (d - 1) (2m + e^{\epsilon} - 1)}{n (m - 1) (e^{\epsilon} - 1)}  } \\ = d \sqrt{l_{2, RR}},
\end{multline}

\noindent regardless of the sample frequency $f$. Same as $l_2$ loss, when
\begin{equation}
    m = 1 + \frac{\Delta}{e^{\epsilon} + d - 1} , \notag
\end{equation}

\noindent where
\begin{equation}
    \Delta = \sqrt{(e^{\epsilon} + d - 1) ( d e^{\epsilon} - e^{\epsilon} + 1)} e^{\epsilon / 2} .\notag
\end{equation}

\noindent The upper bound of $l_1$ loss reaches its minimum, which is
\begin{equation}
    \lceil l_{1} \rceil  = d \sqrt{\frac{2(\Delta + d e^{\epsilon})}{n (e^{\epsilon} - 1)^2}} .
\end{equation}
